DeepChange: A Large Long-Term Person Re-Identification Benchmark with Clothes Change

Existing person re-identification (re-id) works mostly consider short-term application scenarios without clothes change. In real-world, however, we often dress differently across space and time. To solve this contrast, a few recent attempts have been made on long-term re-id with clothes change. Currently, one of the most significant limitations in this field is the lack of a large realistic benchmark. In this work, we contribute a large, realistic long-term person re-identification benchmark, named as DeepChange. It has several unique characteristics: (1) Realistic and rich personal appearance (e.g., clothes and hair style) and variations: Highly diverse clothes change and styles, with varying reappearing gaps in time from minutes to seasons, different weather conditions (e.g., sunny, cloudy, windy, rainy, snowy, extremely cold) and events (e.g., working, leisure, daily activities). (2) Rich camera setups: Raw videos were recorded by 17 outdoor varying resolution cameras operating in a real-world surveillance system. (3) The currently largest number of (17) cameras, (1, 121) identities, and (178, 407) bounding boxes, over the longest time span (12 months). Further, we investigate multimodal fusion strategies for tackling the clothes change challenge. Extensive experiments show that our fusion models outperform a wide variety of state-of-the-art models on DeepChange. Our dataset and documents are available at https://github.com/PengBoXiangShang/deepchange.

==> deepchange-cvpr2022 (4)/tables/comparison-with-cloth-change-datasets.tex <==
\begin{table*}[!t]
  \caption{Comparison with existing long-term image-based re-id datasets with clothes change.
%   including Real28~\cite{wan2020person}, NKUP~\cite{wang2020benchmark}, LTCC~\cite{qian2020long}, PRCC~\cite{yang2019person}. 
  `Fas.': Faster RCNN~\cite{ren2015faster}, `Mas.': Mask RCNN~\cite{he2017mask}, `ind.': indoor, `out.': outdoor, `CD': {\bf cross-day}, `CM': {\bf cross-month}, `CS': {\bf cross-season}, `CY': {\bf cross-year}, `spr.': {\bf spring}, `sum.': {\bf summer}, `aut.': {\bf autumn}, `win.': {\bf winter}, 'sim.': simulated, `sur.': surveillance, '-': unknown.}
  \label{comparison-with-cloth-change-dataset}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l r r r l l l l l l l l | l l l l}
    \hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{\# Person} & \multirow{2}{*}{\# Box} & \multirow{2}{*}{\# Cam} & \multirow{2}{*}{Source} & \multirow{2}{*}{Detector} & \multirow{2}{*}{Scene} & \multicolumn{5}{c|}{Time Range} & \multicolumn{4}{c}{Cloth Style} \\
\cline{8-12} \cline{13-16}
 & & & & & & & course & CD & CM & CS & CY & spr. & sum. & aut. & win. \\

    \hline
    \hline
Real28~\cite{wan2020person} & 28 & 4.3K & 4 & sim. &  Mas. & out., ind. & 3 days & $\checkmark$ & &  & & & $\checkmark$ & & \\

NKUP~\cite{wang2020benchmark} & 107 & 9.7K & 15 & sim. & -  & out., ind. & 4 months & $\checkmark$ & $\checkmark$ & $\checkmark$ & & & & $\checkmark$ & $\checkmark$ \\

LTCC~\cite{qian2020long} & 152 & 17K & 12 & sim. & Mas.  & ind. & 2 months & $\checkmark$ & $\checkmark$ &  & & & $\checkmark$ & & \\
 
PRCC~\cite{yang2019person} & 221 & 33K & 3 & sim. &  - & ind. & - & $\checkmark$ & &  & & & $\checkmark$ & & \\
 
%  & & & & &   & & & & &  & & & & \\
 
%  & & & & &   & & & & &  & & & & \\
 
%  & & & & &   & & & & &  & & & & \\
 \hline
 \hline
\name & {\bf 1,121} & {\bf 178K} & {\bf 17} & {\bf sur.} & Fas.  & out. & {\bf 12 months} & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
    \hline
  \end{tabular}
  }
\end{table*}




% \begin{table}[!t]
%   \caption{Comparison with existing long-term image-based Re-ID datasets with clothes change. (`Fas.': Faster RCNN~\cite{ren2015faster}, `Mas.': Mask RCNN~\cite{he2017mask}, `ind.': indoor, `out.': outdoor, `CD': {\bf cross-day}, `CM': {\bf cross-month}, `CS': {\bf cross-season}, `CY': {\bf cross-year}, `spr.': {\bf spring}, `sum.': {\bf summer}, `aut.': {\bf autumn}, `win.': {\bf winter}, 'sim.': simulated, `sur.': surveillance, '-': unknown)}
%   \label{comparison-with-cloth-change-dataset}
%   \centering
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{l r r r l l l l l l l l l l l l}
%     \hline
    
% \multirow{2}{*}{dataset} & \multirow{2}{*}{\# person} & \multirow{2}{*}{\# bbox} & \multirow{2}{*}{\# cam} & \multirow{2}{*}{source} & \multirow{2}{*}{detector} & \multirow{2}{*}{scene} & \multicolumn{5}{c}{time range} & \multicolumn{4}{c}{cloth style} \\
% \cline{8-12} \cline{13-16}
%  & & & & & & & course & CD & CM & CS & CY & spr. & sum. & aut. & win. \\

%     \hline
%     \hline
% Real28~\cite{wan2020person} & 28 & 4.3K & 4 & sim. &  Mas. & out., ind. & 3 days & $\checkmark$ & &  & & & $\checkmark$ & & \\

% NKUP~\cite{wang2020benchmark} & 107 & 9.7K & 15 & sim. & -  & out., ind. & 4 months & $\checkmark$ & $\checkmark$ & $\checkmark$ & & & & $\checkmark$ & $\checkmark$ \\

% LTCC~\cite{qian2020long} & 152 & 17K & 12 & sim. & Mas.  & ind. & 2 months & $\checkmark$ & $\checkmark$ &  & & & $\checkmark$ & & \\
 
% PRCC~\cite{yang2019person} & 221 & 33K & 3 & sim. &  - & ind. & - & $\checkmark$ & &  & & & $\checkmark$ & & \\
 
% %  & & & & &   & & & & &  & & & & \\
 
% %  & & & & &   & & & & &  & & & & \\
 
% %  & & & & &   & & & & &  & & & & \\
%  \hline
%  \hline
% \name & {\bf 1,121} & {\bf 178K} & {\bf 17} & {\bf sur.} & Fas.  & out. & {\bf 12 months} & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
%     \hline
%   \end{tabular}
%   }
% \end{table}

==> deepchange-cvpr2022 (4)/tables/comparison-with-traditional-datasets.tex <==
\begin{table*}[!t]
  \caption{Comparison with conventional short-term image-based Re-ID datasets without clothes change. (`Fas.': Faster RCNN~\cite{ren2015faster}, `DPM': Deformable Part Model~\cite{felzenszwalb2009object}, `ind.': indoor, `out.': outdoor)}
  \label{comparison-with-traditional-dataset}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l l l l l l l l l l}
    \hline
    
    
Dataset & \name & MSMT17~\cite{wei2018person} & Duke~\cite{zheng2017unlabeled} & Market~\cite{zheng2015scalable} & CUHK03~\cite{li2014deepreid} & CUHK01~\cite{li2012human} & VIPeR~\cite{gray2008viewpoint} & PRID~\cite{hirzer2011person} & CAVIAR~\cite{cheng2011custom} \\

    \hline
    \hline
\# Person & 1,121 & 4,101 & 1,812 & 1,501 & 1,467 & 971 & 632 & 934 & 72 \\
\# Bbox & {\bf 178K} & 126K & 36K & 32K & 28K & 3.8K & 1.2K & 1.1K & 0.6K \\
\# Camera & {\bf 17} & 15 & 8 & 6 & 2 & 10 & 2 & 2 & 2 \\
Detector & Fas. & Fas. & hand & DPM & DPM, hand & hand & hand & hand & hand \\
Scene & out. & out. \& ind. & out. & out. & ind. & ind. & out. & out. & ind. \\
    \hline
  \end{tabular}
  }
\end{table*}

% \begin{table}[!t]
%   \caption{\todo Comparison with conventional short-term image-based Re-ID datasets without clothes change. (`DPM': Deformable Part Model~\cite{felzenszwalb2009object})}
%   \label{comparison-with-traditional-dataset}
%   \centering
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{l r r r l l}
%     \hline
    
    
% dataset & ~~\# person~~ & ~~\# bbox~~ & ~~\# camera~~ & ~~detector~~ & ~~scene \\
% \hline
% \hline
% \name & 1,121 & {\bf 178K} & {\bf 17} & Faster RCNN & outdoor \\
% MSMT17~\cite{wei2018person} & 4,101 & 126K & 15 & Faster RCNN & outdoor, indoor \\
% Duke~\cite{zheng2017unlabeled} & 1,812 & 36K & 8 & hand & outdoor \\
% Market~\cite{zheng2015scalable} & 1,501 & 32K & 6 & DPM & outdoor \\
% CUHK03~\cite{li2014deepreid} & 1,467 & 28K & 2 & DPM, hand & indoor \\
% CUHK01~\cite{li2012human} & 971 & 3.8K &  10 & hand & indoor \\
% VIPeR~\cite{gray2008viewpoint} & 632 & 1.2K & 2 & hand & outdoor \\
% PRID~\cite{hirzer2011person} & 934 & 1.1K &  2 &  hand & outdoor \\
% CAVIAR~\cite{cheng2011custom} & 72 & 0.6K & 2 & hand & indoor \\

%     \hline
%   \end{tabular}
%   }
% \end{table}

==> deepchange-cvpr2022 (4)/tables/dataset-split-table-2-settings.tex <==
\begin{table}[!t]
  \caption{Dataset splitting of \name. \todo two settings}
  \label{dataset-split-table}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l  c c c c c c c}
    \hline
 & \multicolumn{3}{c}{setting \#1} & & \multicolumn{3}{c}{setting \#2} \\    
 \cline{2-4} \cline{6-8}   
 & train set & validation set & test set & & train set & validation set & test set\\
    \hline
    \hline
\# person & 450 & 150 & 521 & & \multicolumn{2}{c}{600 (shared)} & 521\\    
 \multirow{2}{*}{\# bbox} & \multirow{2}{*}{75,083} & probe: 4,976 & probe: 17,527 & & \multirow{2}{*}{88,132} & \multirow{2}{*}{9,792} & probe: 17,527 \\
  &  & gallery: 17,865 & gallery: 62,956 & &   &   & gallery: 62,956 \\

    \hline
  \end{tabular}
  }
\end{table}

==> deepchange-cvpr2022 (4)/tables/dataset-split-table.tex <==
\begin{table}[!t]
  \caption{Dataset splitting of \name.}
  \label{dataset-split-table}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l l l l}
    \hline
    
    
 & Train set & Validation set & Test set \\

    \hline
    \hline
\# Person & 450 & 150 & 521 \\    
\multirow{2}{*}{\# Box} & \multirow{2}{*}{75,083} & Probe: 4,976 & Probe: 17,527 \\
 &  & Gallery: 17,865 & Gallery: 62,956 \\

    \hline
  \end{tabular}
  }
\end{table}

==> deepchange-cvpr2022 (4)/tables/main-results-setting2.tex <==
\begin{table}[!t]
  \caption{\todo setting 2, Person Re-ID performance comparisons on the test set of \name. Both rank accuracy ($\%$) and mAP ($\%$) are reported. (`R': RGB, `G': grayscale, `E': edge map, `K': body key point, `2br': two branches, `3br': three branches) \red{box plots}}
  \label{main-results-setting2}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l l l c c c c c c}
    \hline
    
    
\multirow{2}{*}{network/model} & \multicolumn{2}{c}{input} &  \multirow{2}{*}{batch size} & \multicolumn{4}{c}{rank} & \multirow{2}{*}{mAP} \\
\cline{2-3} \cline{5-8}
 & modalities & dimensions &   & @1 & @5 & @10 & @20 &  \\
    \hline
    \hline
    
\#1 ResNet18~\cite{he2016deep} & R & 256$\times$128  &  256 &     &   &   &   &   \\

\#2 ResNet18~\cite{he2016deep} & G & 256$\times$128  &  256 &  &   &   &   & \\



\#3 ResNet34~\cite{he2016deep} & R & 256$\times$128 &  256  & &   &   &   & \\

\#4 ResNet34~\cite{he2016deep} & G & 256$\times$128  &  256  & &   &   &   & \\



\#5 ResNet50~\cite{he2016deep} & R & 256$\times$128  &  192 &   &    &    &    &   \\
%\#5 ResNet50~\cite{he2016deep} & R & 256$\times$128  &  192 & 38.93 &  50.90 & 56.50  &  62.38 & 10.78 \\

\#6 ResNet50~\cite{he2016deep} & G & 256$\times$128  &  192 & &   &   &   & \\

\#7 ResNet50~\cite{he2016deep} & E & 256$\times$128  &  192 & &   &   &   & \\



\#8 ResNet101~\cite{he2016deep} & R & 256$\times$128  &  128 & 41.24 & 52.98  &  58.89 & 65.53  & 12.04 \\

\#9 ResNet152~\cite{he2016deep} & R & 256$\times$128  &  \red{80} & 42.66 &  54.79 &  60.63 & 66.93  & 12.48 \\
% batch size = 96, CUDA out of memory.

\#10 MobileNetv2~\cite{sandler2018mobilenetv2} & R & 256$\times$128  &  256 & &   &   &   & \\



\#11 Inceptionv3~\cite{Szegedy_2016_CVPR}  & R & 299$\times$299  &  96 &  &   &   &   & \\



\#12 DenseNet121~\cite{huang2017densely} & R & 256$\times$128  &  128 & 39.10 & 50.96  & 56.87  & 62.65  & 09.73 \\
\#12 DenseNet121~\cite{huang2017densely} & G & 256$\times$128  &  128 & \blue{30.63}  &  \blue{42.77}  &  \blue{49.20}  &  \blue{55.69}  & \blue{06.21}  \\
\#12 DenseNet121~\cite{huang2017densely} & E & 256$\times$128  &  128 & 19.25  &  31.31  &  38.04  &  45.63  &  03.11 \\
\#13 DenseNet161~\cite{huang2017densely} & R & 256$\times$128  &  64 & &   &   &   & \\

\#14 DenseNet169~\cite{huang2017densely} & R & 256$\times$128  &  96 & 42.94 & 53.79  & 58.99  & 64.88  & 11.14 \\
      & & & & \red{44.03} & \red{55.15}  & \red{60.11}  & \red{66.41}  & \red{11.59} \\
      \hline
\#15 DenseNet201~\cite{huang2017densely} & R & 256$\times$128  &  64 & 46.62 &  57.19 &  62.64 &  68.28 & 12.24 \\
\hline
\hline
OSNet x1.0~\cite{zhou2021osnet}     & R & 256$\times$128 & 96 & 42.38 & 54.85  & 60.58  & 66.55  & 11.78 \\
OSNet x0.75~\cite{zhou2021osnet}     & R & 256$\times$128 & 160 & 42.96 & 55.13  & 60.45  & 66.20  & 11.13 \\
OSNet x0.5~\cite{zhou2021osnet}     & R & 256$\times$128 & 256 & 41.55 & 54.05  & 59.39  & 65.19  & 10.88 \\
OSNet x0.25~\cite{zhou2021osnet}     & R & 256$\times$128 & 512 & 36.63 & 49.51  & 55.82  &  62.27 & 09.28 \\
\hline
\hline
\#16 ReIDCaps~\cite{huang2019beyond} & R & 224$\times$224  &  \red{20} & 48.55 &  59.94 &  65.26 &  71.18 & 15.34 \\

\#17 2br ResNet50 & R, K & 256$\times$128  &  192 & &   &   &   & \\

\#18 2br ResNet50 & R, E & 256$\times$128  &  96 & &   &   &   & \\

\#19 2br ResNet50 & R, G & 256$\times$128  &  96 &  41.79 & 53.96  & 59.90  & 66.42 & 10.82 \\

\#20 3br ResNet50 & R, G, E & 256$\times$128  &  64 & &   &   &   & \\

\#21 2br DenseNet121 & R, E & 256$\times$128  &  64 & &   &   &   & \\

\#22 2br DenseNet121 & R, G & 256$\times$128  &  64 & &   &   &   & \\

\#23 3br DenseNet121 & R, G, E & 256$\times$128  &  32 & 47.61 &  58.76 &  64.37 & 70.19  & 12.61 \\
    \hline
  \end{tabular}
  }
\end{table}

==> deepchange-cvpr2022 (4)/tables/main-results-v20210726-backup-color.tex <==
\begin{table*}[!h]
\tiny
  \caption{Person Re-ID performance comparisons on the test set of \name. Both rank accuracy ($\%$) and mAP ($\%$) are reported. (`R': RGB, `G': grayscale, `E': edge map, `K': body key point, `2br': two branches, `3br': three branches, `mod.': modalities, `dim.': dimensions)}
  \label{main-results}
  \centering
  %\resizebox{\linewidth}{!}{
  \scalebox{1.3}{
  \begin{tabular}{l l l c c c c c c}
    \hline
    
    
\multirow{2}{*}{network/model} & \multicolumn{2}{c}{input} &  \multirow{2}{*}{batch size} & \multicolumn{4}{c}{rank} & \multirow{2}{*}{mAP} \\
\cline{2-3} \cline{5-8}
 & mod. & dim. &   & @1 & @5 & @10 & @20 &  \\
    \hline
    \hline
% vgg13      & & & & \red{} & \red{}  & \red{}  & \red{}  & \red{} \\
% vgg16      & & & & \red{} & \red{}  & \red{}  & \red{}  & \red{} \\
% vgg19      & & & & \red{} & \red{}  & \red{}  & \red{}  & \red{} \\
% \hline
\#1 ResNet18~\cite{he2016deep} & R & 256$\times$128  &  256 & 34.45    &  46.01 & 51.72  & 58.26  &  08.44 \\

\#2 ResNet18~\cite{he2016deep} & G & 256$\times$128  &  256 &  26.61 & 39.02  & 45.45  &  53.06 &  05.49 \\

% ResNet18~\cite{he2016deep} & tri. & 256x128 R & 1e-4, 0.1/40 & 60 & 256 & 38.93 &  53.54 &  59.93 & 66.47 &  09.89 \\

\#3 ResNet34~\cite{he2016deep} & R & 256$\times$128 &  256  & 35.21 &  47.37 &  53.61 &  60.03 & 09.49 \\

\#4 ResNet34~\cite{he2016deep} & G & 256$\times$128  &  256  & 28.60 & 41.53  &  47.98 & 54.87  & 06.39 \\

% ResNet34~\cite{he2016deep} & tri. & 256x128 R & 1e-4, 0.1/40 & 60 & 128 & 38.78 & 52.88 & 59.44 & 66.20 & 10.54 \\

\#5 ResNet50~\cite{he2016deep} & R & 256$\times$128  &  192 & 36.62 & 49.88  &  55.46 & 61.92  & 09.62 \\

\#6 ResNet50~\cite{he2016deep} & G & 256$\times$128  &  192 & 30.04 & 43.12  & 49.82  & 57.04  & 06.96 \\

\#7 ResNet50~\cite{he2016deep} & E & 256$\times$128  &  192 & 16.05 &  28.51 &  35.59  &  43.28 & 03.17 \\

% ResNet50~\cite{he2016deep} & tri. & 256x128 R & 1e-4, 0.1/40 & 60 & 64 & 36.94 & \red{X} & \red{X} & \red{X} & 09.56 \\

resnext50\_32x4d & R & 256$\times$128 & \red{128} & \red{36.94} & \red{48.87}  & \red{54.55}  & \red{60.50}  & \red{10.09} \\
%\hline
wide\_resnet50\_2 & R & 256$\times$128 & \red{128} & \red{33.68} & \red{45.57}  & \red{51.45}  & \red{57.72}  & \red{08.71} \\

\#8 ResNet101~\cite{he2016deep} & R & 256$\times$128  &  128 & 39.31 & 51.65  & 57.36  & 63.72  & 11.00 \\

resnext101\_32x8d & R & 256$\times$128 & \red{64} & \red{40.93} & \red{52.68}  & \red{58.05}  & \red{64.21}  & \red{11.07} \\
%\hline
wide\_resnet101\_2 & R & 256$\times$128 & \red{64} & \red{34.33} & \red{46.46}  & \red{52.42}  & \red{58.69}  & \red{09.03} \\
%\hline
\#9 ResNet152~\cite{he2016deep} & R & 256$\times$128  &  96 & 39.84 & 52.51  & 58.35  &  64.75 & 11.49 \\

\#10 MobileNetv2~\cite{sandler2018mobilenetv2} & R & 256$\times$128  &  256 & 33.71 & 46.51  & 52.72  & 59.45  & 07.95 \\

% MobileNetv2~\cite{sandler2018mobilenetv2} & tri. & 256x128 R & 1e-4, 0.1/40 & 60 & 96 & 36.85 & 51.96 & 58.73  & 65.51 & 09.35 \\
MobileNetv3 Small~\cite{howard2019searching}     & R & 256$\times$128 & \red{768} & \red{28.73} & \red{40.87}  & \red{47.24}  & \red{54.12}  & \red{06.09} \\
MobileNetv3 Large~\cite{howard2019searching}     & R & 256$\times$128 & \red{320} & \red{33.08} & \red{44.99}  & \red{51.32}  & \red{58.14}  & \red{07.56} \\
%\hline
GoogLeNet      & R & 299$\times$299 & \red{96} & \red{29.02} & \red{40.83}  & \red{46.75}  & \red{53.65}  & \red{07.24} \\
\#11 Inceptionv3~\cite{Szegedy_2016_CVPR}  & R & 299$\times$299  &  96 &  35.02 &  47.71 &  53.91 &  60.64 & 08.85 \\

% Inceptionv3~\cite{Szegedy_2016_CVPR}  & tri. & 299x299 R & 1e-4, 0.1/40 & 60 & 32 & 22.18 & \red{X} & \red{X} & \red{X} & 06.01 \\

{\#12 DenseNet121}~\cite{huang2017densely} & R & 256$\times$128  &  128 & 38.26 & 50.27  &  55.91 &  62.40 & 09.12 \\
{\# DenseNet121}~\cite{huang2017densely} & \red{G} & 256$\times$128  &  128 & \red{30.64} & \red{43.02}  & \red{49.41}  & \red{56.44}  & \red{06.14}  \\
{\# DenseNet121}~\cite{huang2017densely} & \red{E} & 256$\times$128  &  128 &  \red{18.21} & \red{30.40}  & \red{36.86}  & \red{44.04}  & \red{02.88} \\
{\#12 DenseNet121}~\cite{huang2017densely} & R & \red{224$\times$224}  &  \red{64} & \red{39.92}  &  \red{51.76}  &  \red{57.21}  &   \red{62.98} & \red{09.99}  \\
% repeat & & & & \red{39.47} & \red{51.05}  & \red{56.76}  & \red{62.72}  & \red{09.86} \\
\#13 DenseNet161~\cite{huang2017densely} & R & 256$\times$128  &  64 & 45.92 &  56.72 & 61.79  & 67.41  & 12.30 \\
% repeat      & & & & \red{45.57} & \red{56.78}  & \red{61.84}  & \red{67.31}  & \red{12.02} \\
\#14 DenseNet169~\cite{huang2017densely} & R & 256$\times$128  &  96 & 43.40 &  54.80 &  60.11 &  65.90 & 11.25 \\

\#15 DenseNet201~\cite{huang2017densely} & R & 256$\times$128  &  64 & 44.98 & 56.13  & 61.32  & 66.98  & 11.71 \\
%\hline
%\hline
shufflenetv2\_x0.5      & R & 256$\times$128 & \red{1024} & \red{17.21} & \red{27.69}  & \red{33.48}  & \red{40.53}  & \red{04.00} \\
shufflenetv2\_x1.0      & R & 256$\times$128 & \red{768} & \red{20.22} & \red{32.95}  & \red{39.58}  & \red{46.89}  & \red{04.60} \\
%\hline
squeezenet1\_0      & R & 256$\times$128 & \red{384} & \red{23.38} & \red{33.17}  & \red{38.64}  & \red{44.34}  & \red{04.78} \\
squeezenet1\_1      & R & 256$\times$128 & \red{640} & \red{23.52} & \red{33.54}  & \red{39.26}  & \red{45.59}  & \red{05.02} \\
%\hline
mnasnet0\_5 & R & 256$\times$128 & 512 & \red{17.52} & \red{29.17}  & \red{36.20}  & \red{43.51}  & \red{02.79} \\
mnasnet1\_0 & R & 256$\times$128 & \red{256} & \red{30.63} & \red{44.02}  & \red{50.40}  & \red{57.56}  & \red{06.25} \\
\hline
SCNet50~\cite{liu2020improving}      & R & 256$\times$128 & \red{160} & \red{35.07} & \red{47.73}  & \red{54.32}  & \red{60.73}  & \red{09.53} \\
SCNet50\_v1d~\cite{liu2020improving}      & R & 256$\times$128 & \red{128} & \red{37.46} & \red{50.20}  & \red{56.13}  & \red{62.36}  & \red{09.42} \\
SCNet101~\cite{liu2020improving}      & R & 256$\times$128 & \red{96} & \red{37.25} & \red{50.09}  & \red{56.28}  & \red{63.16}  & \red{10.35} \\
\hline
%\hline
OSNet ibn x1.0~\cite{zhou2021osnet} & R & 256$\times$128 & \red{96} & \red{42.75} & \red{54.91}  & \red{60.82}  & \red{66.80}  & \red{10.97} \\
OSNet x1.0~\cite{zhou2021osnet}     & R & 256$\times$128 & 96 & \red{39.65} & \red{52.22}  & \red{58.32}  & \red{64.23}  & \red{10.34} \\
OSNet x0.75~\cite{zhou2021osnet}     & R & 256$\times$128 & 160 & \red{39.96} & \red{51.89}  & \red{57.69}  & \red{63.85}  & \red{09.92} \\
OSNet x0.5~\cite{zhou2021osnet}     & R & 256$\times$128 & 256 & \red{38.09} & \red{51.08}  & \red{56.79}  & \red{63.27}  & \red{09.59} \\
OSNet x0.25~\cite{zhou2021osnet}     & R & 256$\times$128 & 512 & \red{34.94} & \red{47.70}  & \red{54.10}  & \red{60.77}  & \red{08.62} \\
%OSNet & CE & 256x128 & 1e-4, 0.1 per 20 & 30 & 96 & 0.4464 & 0.5680 & 0.6247 & 0.6806 & 0.1100 \\
\hline
BNNeck Re-ID Res18~\cite{luo2020strong}     & R & 256$\times$128 & \red{224} & \blue{38.17} & \red{51.93}  & \red{58.08}  & \red{64.70}  & \red{09.51} \\
BNNeck ResNet34~\cite{luo2020strong}     & R & 256$\times$128 & \red{128} & \red{40.06} & \red{53.49}  & \red{59.55}  & \red{66.25}  & \red{10.52} \\
BNNeck ResNet50~\cite{luo2020strong}      & R & 256$\times$128 & \red{56} & \red{47.45} & \red{59.47}  & \red{65.19}  & \red{71.10}  & \red{12.98} \\
\hdashline
BNNeck ResNet50~\cite{luo2020strong}      & G & 256$\times$128 & \red{56} & \red{4002} & \red{5404}  & \red{6019}  & \red{6709}  & \red{0943} \\
BNNeck ResNet50~\cite{luo2020strong}      & E & 256$\times$128 & \red{56} & \red{2175} & \red{3599}  & \red{4311}  & \red{5081}  & \red{0367} \\
2br BNNeck ResNet50~\cite{luo2020strong}      & R, G & 256$\times$128 & \blue{28} & \red{46.62} & \red{59.72}  & \red{65.58}  & \red{71.48}  & \red{13.12} \\
BNNeck ResNet50~\cite{luo2020strong}      & R, G, E & 256$\times$128 & \red{56} & \red{} & \red{}  & \red{}  & \red{}  & \red{} \\
\hdashline
BNNeck ResNet101~\cite{luo2020strong}     & R & 256$\times$128 & \red{40} & \red{48.10} & \red{60.70}  & \red{66.10}  & \red{72.06}  & \red{13.72} \\
BNNeck ResNet152~\cite{luo2020strong}     & R & 256$\times$128 & & \green{50.29} & \red{62.27}  & \red{67.85}  & \red{73.63}  & \green{14.59} \\
BNNeck Re-ID Den121     & R & 256$\times$128 & & \green{4786} & \red{6047}  & \red{6588}  & \red{7164}  & \green{1341} \\
\hline
\tabincell{c}{\#16 ReIDCaps~\cite{huang2019beyond}\\ (full model)} & R & 224$\times$224  &  24 & 44.29 & 56.44  & 62.01  & 68.01  & 13.25 \\
% repeat & & & & \red{44.49} & \red{56.32}  & \red{61.80}  & \red{68.21}  & \red{13.28} \\
% repeat  & & & & \red{44.97} & \red{56.35}  & \red{61.99}  & \red{68.01}  & \red{13.29} \\
% repeat  & & & & \red{43.88} & \red{56.18}  & \red{61.98}  & \red{67.77}  & \red{13.03} \\
\tabincell{c}{\#16 ReIDCaps~\cite{huang2019beyond}\\ (full model, resnet50 backbone)} & R & \red{224$\times$224}  &  \red{32} & \red{3949} & \red{5228}  &  \red{5868} & \red{6499}  & \red{1133} \\
   \hline
\tabincell{c}{\#16 ReIDCaps~\cite{huang2019beyond}\\(no auxiliary module\&loss)} & R & 224$\times$224  &  24 & \red{35.41} & \red{46.66}  & \red{52.09}  & \red{58.13}  & \red{09.25} \\
% repeat & & & & \red{34.97} & \red{46.23}  & \red{51.80}  & \red{58.26}  & \red{09.33} \\
 \hline
\tabincell{c}{\#16 ReIDCaps~\cite{huang2019beyond}\\ (no capsule module\&loss)} & R & \red{224$\times$224}  &  80 & \red{39.38} & \red{51.86}  & \red{57.82}  & \red{64.44}  & \red{11.16} \\
% repeat & & & & \red{39.94} & \red{52.22}  & \red{57.73}  & \red{64.14}  & \red{11.36} \\
%\#16 ReIDCaps~\cite{huang2019beyond} & R & \red{256$\times$128}  &  24 & \red{x} & \red{x}  & \red{x}  & \red{x}  & \red{x} \\
\hline
\#17 2br ResNet50 & R, K & 256$\times$128  &  192 & 36.53 &  48.87 &  54.86 &  61.47 & 09.54 \\

\#18 2br ResNet50 & R, E & 256$\times$128  &  96 & 40.26 & 52.91  & 59.11  & 65.47  & 10.43 \\

\#19 2br ResNet50 & R, G & 256$\times$128  &  96 & 40.52 &  53.65  &  59.61 &  65.60 & 10.22 \\

\#20 3br ResNet50 & R, G, E & 256$\times$128  &  64 & 41.67 & 54.28  & 60.04   &  66.37 & 11.03 \\

\#21 2br DenseNet121 & R, E & 256$\times$128  &  64 & 44.55 & 56.40  &  62.03 &  67.85 & 11.21 \\

\#22 2br DenseNet121 & R, G & 256$\times$128  &  64 & 44.80 &  56.79 &  62.48 & 68.06  & 11.36 \\
\hline
\#23 3br DenseNet121 & R, G, E & 256$\times$128  &  32 & 45.36 & 57.36  & 62.91  & 69.29  & 11.73 \\
%  repeat & & & & \red{44.87} & \red{57.14}  & \red{63.12}  & \red{69.26}  & \red{11.36} \\
%  repeat & & & & \red{45.36} & \red{57.36}  & \red{62.91}  & \red{69.29}  & \red{11.73} \\
%  repeat & & & & \red{44.75} & \red{56.80}  & \red{62.60}  & \red{68.34}  & \red{11.54} \\
%  repeat   & & & & \red{46.00} & \red{58.24}  & \red{63.80}  & \red{69.61}  & \red{11.76} \\
%  repeat    & & & & \red{45.06} & \red{57.66}  & \red{63.32}  & \red{69.30}  & \red{11.86} \\
%  repeat     & & & & \red{46.09} & \red{58.43}  & \red{63.77}  & \red{69.85}  & \red{11.87} \\     
%  repeat    & & & & \red{} & \red{}  & \red{}  & \red{}  & \red{} \\
    \hline
    \hline
%ViT B16~\cite{dosovitskiy2020image} & R & \red{224$\times$224} & 128 4GPUs & \red{38.90} & \red{50.79} & \red{56.25} & \red{62.47} & \red{11.11} \\ 
ViT B16~\cite{dosovitskiy2020image} & R & \red{256$\times$128} & 128 4GPUs & \red{41.30} & \red{53.83} & \red{59.44} & \red{65.44} & \red{12.04} \\ % ImageNet21K, class token,
      & R & & 64 1GPU & \red{43.96} & \red{55.82}  & \red{61.22}  & \red{66.74}  & \red{12.98} \\ %    ImageNet21K, class token,  learning rate decay changes.
            & R & & 64 1GPU & \red{49.78} & \red{61.81}  & \red{67.38}  & \red{72.92}  & \red{14.98} \\ % ImageNet21K+ImageNet1K, mean tokens, no layer norm,
                  & Gray & & 64 1GPU & \red{38.93} & \red{51.94}  & \red{58.50}  & \red{65.12}  & \red{10.43} \\ % ImageNet21K+ImageNet1K, mean tokens, no layer norm,
%      & Gray & & 64 1GPU & \red{} & \red{}  & \red{}  & \red{}  & \red{} \\ %ImageNet21K+ImageNet1K, mean tokens, +layer norm,
\hline
ViT B16 0.3* Gray+1* RGB    & R, G & \red{256$\times$256} & 64 1GPU  & \red{0.4725} & \red{0.5852} & \red{0.6366} & \red{0.6936} & \red{0.1470} \\ % 3* Gray+1* RGB
ViT B16 0.3* Gray+0.7* RGB    & R, G & \red{256$\times$256} & 64 1GPU & \red{0.4724} & \red{0.5853} & \red{0.6407} & \red{0.6953} & \red{0.1463} \\ % 0.3* Gray+0.7* RGB
\hline
DeiT     & R & 256$\times$128 & 64 1GPU & \blue{0.4443} & \blue{0.5625} & \blue{0.6182} & \blue{0.6746} & \blue{0.1372} \\
%DeiT      & & & & \red{} & \red{}  & \red{}  & \red{}  & \red{} \\
    \hline
  \end{tabular}
  }
\end{table*}

==> deepchange-cvpr2022 (4)/tables/main-results-v20210726-table1.tex <==
\begin{table*}[!t]
\tiny
  \caption{{Unimodal results} on the test set of \name. Both rank accuracy ($\%$) and mAP ($\%$) are reported. (`R': RGB, `G': Grayscale, `E': Edge map, `K': Body key point, `Mod.': Modalities)}
  \label{table:baselines}
  \centering
  \resizebox{\linewidth}{!}{
  %\scalebox{1.3}{
  \begin{tabular}{l l l c c c c c c}
    \hline
    
    
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Input} &  \multirow{2}{*}{Batch size} & \multicolumn{4}{c}{Rank} & \multirow{2}{*}{mAP} \\
\cline{2-3} \cline{5-8}
 & Mod. & Resolution &   & @1 & @5 & @10 & @20 &  \\
    \hline
    \hline
% vgg13      & & & & {} & {}  & {}  & {}  & {} \\
% vgg16      & & & & {} & {}  & {}  & {}  & {} \\
% vgg19      & & & & {} & {}  & {}  & {}  & {} \\
% \hline
\#1 ResNet18~\cite{he2016deep} & R & 256$\times$128  &  256 & 34.45    &  46.01 & 51.72  & 58.26  &  08.44 \\

\#2 ResNet18~\cite{he2016deep} & G & 256$\times$128  &  256 &  26.61 & 39.02  & 45.45  &  53.06 &  05.49 \\

% ResNet18~\cite{he2016deep} & tri. & 256x128 R & 1e-4, 0.1/40 & 60 & 256 & 38.93 &  53.54 &  59.93 & 66.47 &  09.89 \\

\#3 ResNet34~\cite{he2016deep} & R & 256$\times$128 &  256  & 35.21 &  47.37 &  53.61 &  60.03 & 09.49 \\

\#4 ResNet34~\cite{he2016deep} & G & 256$\times$128  &  256  & 28.60 & 41.53  &  47.98 & 54.87  & 06.39 \\

% ResNet34~\cite{he2016deep} & tri. & 256x128 R & 1e-4, 0.1/40 & 60 & 128 & 38.78 & 52.88 & 59.44 & 66.20 & 10.54 \\

\#5 ResNet50~\cite{he2016deep} & R & 256$\times$128  &  192 & 36.62 & 49.88  &  55.46 & 61.92  & 09.62 \\

\#6 ResNet50~\cite{he2016deep} & G & 256$\times$128  &  192 & 30.04 & 43.12  & 49.82  & 57.04  & 06.96 \\

\#7 ResNet50~\cite{he2016deep} & E & 256$\times$128  &  192 & 16.05 &  28.51 &  35.59  &  43.28 & 03.17 \\

% ResNet50~\cite{he2016deep} & tri. & 256x128 R & 1e-4, 0.1/40 & 60 & 64 & 36.94 & {X} & {X} & {X} & 09.56 \\

\#8 ResNext50\_32x4d~\cite{he2016deep} & R & 256$\times$128 & {128} & {36.94} & {48.87}  & {54.55}  & {60.50}  & {10.09} \\
%\hline
\#9 Wide\_ResNet50\_2~\cite{he2016deep} & R & 256$\times$128 & {128} & {33.68} & {45.57}  & {51.45}  & {57.72}  & {08.71} \\

\#10 ResNet101~\cite{he2016deep} & R & 256$\times$128  &  128 & 39.31 & 51.65  & 57.36  & 63.72  & 11.00 \\

\#11 ResNext101\_32x8d~\cite{he2016deep} & R & 256$\times$128 & {64} & {40.93} & {52.68}  & {58.05}  & {64.21}  & {11.07} \\
%\hline
\#12 Wide\_ResNet101\_2~\cite{he2016deep} & R & 256$\times$128 & {64} & {34.33} & {46.46}  & {52.42}  & {58.69}  & {09.03} \\
%\hline
\#13 ResNet152~\cite{he2016deep} & R & 256$\times$128  &  96 & 39.84 & 52.51  & 58.35  &  64.75 & 11.49 \\

\#14 MobileNetv2~\cite{sandler2018mobilenetv2} & R & 256$\times$128  &  256 & 33.71 & 46.51  & 52.72  & 59.45  & 07.95 \\

% MobileNetv2~\cite{sandler2018mobilenetv2} & tri. & 256x128 R & 1e-4, 0.1/40 & 60 & 96 & 36.85 & 51.96 & 58.73  & 65.51 & 09.35 \\
\#15 MobileNetv3 Small~\cite{howard2019searching}     & R & 256$\times$128 & {768} & {28.73} & {40.87}  & {47.24}  & {54.12}  & {06.09} \\
\#16 MobileNetv3 Large~\cite{howard2019searching}     & R & 256$\times$128 & {320} & {33.08} & {44.99}  & {51.32}  & {58.14}  & {07.56} \\
%\hline
\#17 GoogLeNet~\cite{szegedy2015going}      & R & 299$\times$299 & {96} & {29.02} & {40.83}  & {46.75}  & {53.65}  & {07.24} \\
\#18 Inceptionv3~\cite{Szegedy_2016_CVPR}  & R & 299$\times$299  &  96 &  35.02 &  47.71 &  53.91 &  60.64 & 08.85 \\

% Inceptionv3~\cite{Szegedy_2016_CVPR}  & tri. & 299x299 R & 1e-4, 0.1/40 & 60 & 32 & 22.18 & {X} & {X} & {X} & 06.01 \\

{\#19 DenseNet121}~\cite{huang2017densely} & R & 256$\times$128  &  128 & 38.26 & 50.27  &  55.91 &  62.40 & 09.12 \\
{\#20 DenseNet121}~\cite{huang2017densely} & {G} & 256$\times$128  &  128 & {30.64} & {43.02}  & {49.41}  & {56.44}  & {06.14}  \\
{\#21 DenseNet121}~\cite{huang2017densely} & {E} & 256$\times$128  &  128 &  {18.21} & {30.40}  & {36.86}  & {44.04}  & {02.88} \\
{\#22 DenseNet121}~\cite{huang2017densely} & R & {224$\times$224}  &  {64} & {39.92}  &  {51.76}  &  {57.21}  &   {62.98} & {09.99}  \\
% repeat & & & & {39.47} & {51.05}  & {56.76}  & {62.72}  & {09.86} \\
\#23 DenseNet161~\cite{huang2017densely} & R & 256$\times$128  &  64 & 45.92 &  56.72 & 61.79  & 67.41  & 12.30 \\
% repeat      & & & & {45.57} & {56.78}  & {61.84}  & {67.31}  & {12.02} \\
\#24 DenseNet169~\cite{huang2017densely} & R & 256$\times$128  &  96 & 43.40 &  54.80 &  60.11 &  65.90 & 11.25 \\

\#25 DenseNet201~\cite{huang2017densely} & R & 256$\times$128  &  64 & 44.98 & 56.13  & 61.32  & 66.98  & 11.71 \\
%\hline
%\hline
\#26 ShuffleNetv2\_x0.5~\cite{ma2018shufflenet}      & R & 256$\times$128 & {1024} & {17.21} & {27.69}  & {33.48}  & {40.53}  & {04.00} \\
\#27 ShuffleNetv2\_x1.0~\cite{ma2018shufflenet}      & R & 256$\times$128 & {768} & {20.22} & {32.95}  & {39.58}  & {46.89}  & {04.60} \\
%\hline
\#28 SqueezeNet1\_0~\cite{iandola2016squeezenet}      & R & 256$\times$128 & {384} & {23.38} & {33.17}  & {38.64}  & {44.34}  & {04.78} \\
\#29 SqueezeNet1\_1~\cite{iandola2016squeezenet}      & R & 256$\times$128 & {640} & {23.52} & {33.54}  & {39.26}  & {45.59}  & {05.02} \\
%\hline
\#30 MnasNet0\_5~\cite{tan2019mnasnet} & R & 256$\times$128 & 512 & {17.52} & {29.17}  & {36.20}  & {43.51}  & {02.79} \\
\#31 MnasNet1\_0~\cite{tan2019mnasnet} & R & 256$\times$128 & {256} & {30.63} & {44.02}  & {50.40}  & {57.56}  & {06.25} \\
\hline
\hline
\#32 SCNet50~\cite{liu2020improving}      & R & 256$\times$128 & {160} & {35.07} & {47.73}  & {54.32}  & {60.73}  & {09.53} \\
\#33 SCNet50\_v1d~\cite{liu2020improving}      & R & 256$\times$128 & {128} & {37.46} & {50.20}  & {56.13}  & {62.36}  & {09.42} \\
\#34 SCNet101~\cite{liu2020improving}      & R & 256$\times$128 & {96} & {37.25} & {50.09}  & {56.28}  & {63.16}  & {10.35} \\
\hline
\hline
\#35 OSNet ibn x1.0~\cite{zhou2021osnet} & R & 256$\times$128 & {96} & {42.75} & {54.91}  & {60.82}  & {66.80}  & {10.97} \\
\#36 OSNet x1.0~\cite{zhou2021osnet}     & R & 256$\times$128 & 96 & {39.65} & {52.22}  & {58.32}  & {64.23}  & {10.34} \\
\#37 OSNet x0.75~\cite{zhou2021osnet}     & R & 256$\times$128 & 160 & {39.96} & {51.89}  & {57.69}  & {63.85}  & {09.92} \\
\#38 OSNet x0.5~\cite{zhou2021osnet}     & R & 256$\times$128 & 256 & {38.09} & {51.08}  & {56.79}  & {63.27}  & {09.59} \\
\#39 OSNet x0.25~\cite{zhou2021osnet}     & R & 256$\times$128 & 512 & {34.94} & {47.70}  & {54.10}  & {60.77}  & {08.62} \\
%OSNet & CE & 256x128 & 1e-4, 0.1 per 20 & 30 & 96 & 0.4464 & 0.5680 & 0.6247 & 0.6806 & 0.1100 \\

\#40 BNNeck \reid{} ResNet18~\cite{luo2020strong}     & R & 256$\times$128 & {224} & {38.17} & {51.93}  & {58.08}  & {64.70}  & {09.51} \\
\#41 BNNeck \reid{} ResNet34~\cite{luo2020strong}     & R & 256$\times$128 & {128} & {40.06} & {53.49}  & {59.55}  & {66.25}  & {10.52} \\
\#42 BNNeck \reid{} ResNet50~\cite{luo2020strong}      & R & 256$\times$128 & {56} & {47.45} & {59.47}  & {65.19}  & {71.10}  & {12.98} \\
%\hdashline
\#43 BNNeck \reid{} ResNet50~\cite{luo2020strong}      & G & 256$\times$128 & {56} & {40.02} & {54.04}  & {60.19}  & {67.09}  & {09.43} \\
\#44 BNNeck \reid{} ResNet50~\cite{luo2020strong}      & E & 256$\times$128 & {56} & {21.75} & {35.99}  & {43.11}  & {50.81}  & {03.67} \\
% \#45 2br BNNeck ResNet50~\cite{luo2020strong}      & R, G & 256$\times$128 & {28} & {46.62} & {59.72}  & {65.58}  & {71.48}  & {13.12} \\
% \#46 BNNeck ResNet50~\cite{luo2020strong}      & R, G, E & 256$\times$128 & {56} & {} & {}  & {}  & {}  & {} \\
%\hdashline
\#45 BNNeck \reid{} ResNet101~\cite{luo2020strong}     & R & 256$\times$128 & {40} & {48.10} & {60.70}  & {66.10}  & {72.06}  & {13.72} \\
\#46 BNNeck \reid{} ResNet152~\cite{luo2020strong}     & R & 256$\times$128 & 28 & {50.29} & {62.27}  & {67.85}  & {73.63}  & {14.59} \\
\#47 BNNeck \reid{} DenseNet121~\cite{luo2020strong}     & R & 256$\times$128 & 40 & {47.86} & {60.47}  & {65.88}  & {71.64}  & {13.41} \\
\hline
\hline
\#48 ReIDCaps~\cite{huang2019beyond} (DenseNet121) & R & 224$\times$224  &  24 & 44.29 & 56.44  & 62.01  & 68.01  & 13.25 \\
% repeat & & & & {44.49} & {56.32}  & {61.80}  & {68.21}  & {13.28} \\
% repeat  & & & & {44.97} & {56.35}  & {61.99}  & {68.01}  & {13.29} \\
% repeat  & & & & {43.88} & {56.18}  & {61.98}  & {67.77}  & {13.03} \\
\#49 ReIDCaps~\cite{huang2019beyond} (ResNet50) & R & {224$\times$224}  &  {32} & {39.49} & {52.28}  &  {58.68} & {64.99}  & {11.33} \\
   
{\#50 ReIDCaps~\cite{huang2019beyond} (no auxiliary)} & R & 224$\times$224  &  24 & {35.41} & {46.66}  & {52.09}  & {58.13}  & {09.25} \\
% repeat & & & & {34.97} & {46.23}  & {51.80}  & {58.26}  & {09.33} \\
 
{\#51 ReIDCaps~\cite{huang2019beyond} (no capsule)} & R & {224$\times$224}  &  80 & {39.38} & {51.86}  & {57.82}  & {64.44}  & {11.16} \\
% repeat & & & & {39.94} & {52.22}  & {57.73}  & {64.14}  & {11.36} \\
%\#16 ReIDCaps~\cite{huang2019beyond} & R & {256$\times$128}  &  24 & {x} & {x}  & {x}  & {x}  & {x} \\
\hline
\hline
% \#52 ViT B16~\cite{dosovitskiy2020image}  \todo    & R & {256$\times$128} & 64 & {43.96} & {55.82}  & {61.22}  & {66.74}  & {12.98} \\ %    ImageNet21K, class token,  learning rate decay changes.

\#52 ViT B16~\cite{dosovitskiy2020image}            & R & {256$\times$128} & 64 & {49.78} & {61.81}  & {67.38}  & {72.92}  & {\bf 14.98} \\ % ImageNet21K+ImageNet1K, mean tokens, no layer norm,
% \#53 ViT B16~\cite{dosovitskiy2020image}                  & G\cut{ray} & {256$\times$128} & 64 & {38.93} & {51.94}  & {58.50}  & {65.12}  & {10.43} \\ % ImageNet21K+ImageNet1K, mean tokens, no layer norm,
%      & Gray & & 64 1GPU & {} & {}  & {}  & {}  & {} \\ %ImageNet21K+ImageNet1K, mean tokens, +layer norm,

\#53 ViT B16~\cite{dosovitskiy2020image}                  & G\cut{ray} & {256$\times$128} & 64 & 38.52 & 51.85 & 58.32 & 65.12 & 10.63 \\

\#54 DeiT~\cite{touvron2021training}     & R & 256$\times$128 & 64 & {44.43} & {56.25} & {61.82} & {67.46} & {13.72} \\
    \hline
  \end{tabular}
  }
\end{table*}

==> deepchange-cvpr2022 (4)/tables/main-results-v20210726-table2.tex <==
\begin{table*}[!t]
\tiny
  \caption{{Multimodal results} on the test set of \name. Both rank accuracy ($\%$) and mAP ($\%$) are reported. (`R': RGB, `G': Grayscale, `E': Edge map, `K': Body key point, `2br': Two branches, `3br': Three branches, `Mod.': Modalities, `Dim.': Dimensions)}
  \label{table:multi-modal-baselines}
  \centering
  \resizebox{\linewidth}{!}{
  %\scalebox{1.3}{
  \begin{tabular}{l l l c c c c c c}
    \hline
    
    
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Input} &  \multirow{2}{*}{Batch size} & \multicolumn{4}{c}{Rank} & \multirow{2}{*}{mAP} \\
\cline{2-3} \cline{5-8}
 & Mod. & Dim. &   & @1 & @5 & @10 & @20 &  \\
    \hline
    \hline



\#55 2br ResNet50 & R, K & 256$\times$128  &  192 & 36.53 &  48.87 &  54.86 &  61.47 & 09.54 \\

\#56 2br ResNet50 & R, E & 256$\times$128  &  96 & 40.26 & 52.91  & 59.11  & 65.47  & 10.43 \\

\#57 2br ResNet50 & R, G & 256$\times$128  &  96 & 40.52 &  53.65  &  59.61 &  65.60 & 10.22 \\

\#58 3br ResNet50 & R, G, E & 256$\times$128  &  64 & 41.67 & 54.28  & 60.04   &  66.37 & 11.03 \\

\hline
\hline

\#59 2br DenseNet121 & R, E & 256$\times$128  &  64 & 44.55 & 56.40  &  62.03 &  67.85 & 11.21 \\

\#60 2br DenseNet121 & R, G & 256$\times$128  &  64 & 44.80 &  56.79 &  62.48 & 68.06  & 11.36 \\

\#61 3br DenseNet121 & R, G, E & 256$\times$128  &  32 & 45.36 & 57.36  & 62.91  & 69.29  & 11.73 \\
%  repeat & & & & {44.87} & {57.14}  & {63.12}  & {69.26}  & {11.36} \\
%  repeat & & & & {45.36} & {57.36}  & {62.91}  & {69.29}  & {11.73} \\
%  repeat & & & & {44.75} & {56.80}  & {62.60}  & {68.34}  & {11.54} \\
%  repeat   & & & & {46.00} & {58.24}  & {63.80}  & {69.61}  & {11.76} \\
%  repeat    & & & & {45.06} & {57.66}  & {63.32}  & {69.30}  & {11.86} \\
%  repeat     & & & & {46.09} & {58.43}  & {63.77}  & {69.85}  & {11.87} \\     
%  repeat    & & & & {} & {}  & {}  & {}  & {} \\
    \hline
    \hline
\#62 2br BNNeck \reid{} ResNet50~\cite{luo2020strong}      & R, G & 256$\times$128 & {28} & {46.62} & {59.72}  & {65.58}  & {71.48}  & {13.12} \\
%\#46 BNNeck ResNet50~\cite{luo2020strong}      & R, G, E & 256$\times$128 & {56} & {} & {}  & {}  & {}  & {} \\
    
    

%ViT B16~\cite{dosovitskiy2020image} & R & {224$\times$224} & 128 4GPUs & {38.90} & {50.79} & {56.25} & {62.47} & {11.11} \\ 
% ViT B16~\cite{dosovitskiy2020image} & R & {256$\times$128} & 128 4GPUs & {41.30} & {53.83} & {59.44} & {65.44} & {12.04} \\ % ImageNet21K, class token,
% ViT B16~\cite{dosovitskiy2020image}      & R & {256$\times$128} & 64 & {43.96} & {55.82}  & {61.22}  & {66.74}  & {12.98} \\ %    ImageNet21K, class token,  learning rate decay changes.
% \#63 ViT B16~\cite{dosovitskiy2020image}            & R & {256$\times$128} & 64 & {49.78} & {61.81}  & {67.38}  & {72.92}  & {14.98} \\ % ImageNet21K+ImageNet1K, mean tokens, no layer norm,
% \#64 ViT B16~\cite{dosovitskiy2020image}                  & G\cut{ray} & {256$\times$128} & 64 & {38.93} & {51.94}  & {58.50}  & {65.12}  & {10.43} \\ % ImageNet21K+ImageNet1K, mean tokens, no layer norm,
% %      & Gray & & 64 1GPU & {} & {}  & {}  & {}  & {} \\ %ImageNet21K+ImageNet1K, mean tokens, +layer norm,
\hline
\hline

% \#63 ViT B16 \todo{}* Gray+\todo{}* RGB    & R, G & {256$\times$256} & 64  & 49.98 & 61.67 & 66.88 & 72.44 & 15.68 \\

\#63 \cut{2br} ViT B16~\cite{dosovitskiy2020image}    & 1* R + 0.1 * G      &  256$\times$128  &  32 & {47.83} &59.29&64.59&70.23&15.13\\
% \#27 \cut{2br} VIT~\cite{dosovitskiy2020image}    & 1* R + 1 * G      &  256$\times$128  &  32&46.76&58.17&63.33&69.22&14.80\\
\#64 \cut{2br} ViT B16~\cite{dosovitskiy2020image}    & 1* R + 0.3 * G      &  256$\times$128  &  32& {48.00} &59.47&64.65&70.04& {\bf 15.19} \\

% \#63 ViT B16 0.3* Gray+1* RGB    & R, G & {256$\times$256} & 64  & {0.4725} & {0.5852} & {0.6366} & {0.6936} & {0.1470} \\ % 3* Gray+1* RGB
% \#64 ViT B16 0.3* Gray+0.7* RGB    & R, G & {256$\times$256} & 64 & {0.4724} & {0.5853} & {0.6407} & {0.6953} & {0.1463} \\ % 0.3* Gray+0.7* RGB
% \hline
% DeiT~\cite{touvron2021training}     & R & 256$\times$128 & 64 1GPU & \blue{0.4443} & \blue{0.5625} & \blue{0.6182} & \blue{0.6746} & \blue{0.1372} \\
    \hline
  \end{tabular}
  }
\end{table*}

==> deepchange-cvpr2022 (4)/tables/unsupervised-results.tex <==
\begin{table}[!t]
  \caption{Unsupervised results.}
  \label{unsupervised-results}
  \centering
  \resizebox{0.5\linewidth}{!}{
  \begin{tabular}{l l l l l l}
    \hline
    
    
\multirow{2}{*}{method/model} &  \multicolumn{4}{c}{rank} & \multirow{2}{*}{mAP} \\
\cline{2-5}
    & @1 & @5 & @10 & @20 &  \\

    \hline
    \hline
\#1  xx & xx & xx & xx & xx & xx \\    
\#2  xx & xx & xx & xx & xx & xx \\
\#3  xx & xx & xx & xx & xx & xx \\
\#4  xx & xx & xx & xx & xx & xx \\
\#5  xx & xx & xx & xx & xx & xx \\
\#6  xx & xx & xx & xx & xx & xx \\
%\#7  xx & xx & xx & xx & xx & xx \\
    \hline
  \end{tabular}
  }
\end{table}

==> tables/dataset-split-table-2-settings.tex <==
\begin{table}[!t]
  \caption{Dataset splitting of \name. \todo two settings}
  \label{dataset-split-table}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l  c c c c c c c}
    \hline
 & \multicolumn{3}{c}{setting \#1} & & \multicolumn{3}{c}{setting \#2} \\    
 \cline{2-4} \cline{6-8}   
 & train set & validation set & test set & & train set & validation set & test set\\
    \hline
    \hline
\# person & 450 & 150 & 521 & & \multicolumn{2}{c}{600 (shared)} & 521\\    
 \multirow{2}{*}{\# bbox} & \multirow{2}{*}{75,083} & probe: 4,976 & probe: 17,527 & & \multirow{2}{*}{88,132} & \multirow{2}{*}{9,792} & probe: 17,527 \\
  &  & gallery: 17,865 & gallery: 62,956 & &   &   & gallery: 62,956 \\

    \hline
  \end{tabular}
  }
\end{table}

==> tables/main-results-setting2.tex <==
\begin{table}[!t]
  \caption{\todo setting 2, Person Re-ID performance comparisons on the test set of \name. Both rank accuracy ($\%$) and mAP ($\%$) are reported. (`R': RGB, `G': grayscale, `E': edge map, `K': body key point, `2br': two branches, `3br': three branches) \red{box plots}}
  \label{main-results-setting2}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l l l c c c c c c}
    \hline
    
    
\multirow{2}{*}{network/model} & \multicolumn{2}{c}{input} &  \multirow{2}{*}{batch size} & \multicolumn{4}{c}{rank} & \multirow{2}{*}{mAP} \\
\cline{2-3} \cline{5-8}
 & modalities & dimensions &   & @1 & @5 & @10 & @20 &  \\
    \hline
    \hline
    
\#1 ResNet18~\cite{he2016deep} & R & 256$\times$128  &  256 &     &   &   &   &   \\

\#2 ResNet18~\cite{he2016deep} & G & 256$\times$128  &  256 &  &   &   &   & \\



\#3 ResNet34~\cite{he2016deep} & R & 256$\times$128 &  256  & &   &   &   & \\

\#4 ResNet34~\cite{he2016deep} & G & 256$\times$128  &  256  & &   &   &   & \\



\#5 ResNet50~\cite{he2016deep} & R & 256$\times$128  &  192 &   &    &    &    &   \\
%\#5 ResNet50~\cite{he2016deep} & R & 256$\times$128  &  192 & 38.93 &  50.90 & 56.50  &  62.38 & 10.78 \\

\#6 ResNet50~\cite{he2016deep} & G & 256$\times$128  &  192 & &   &   &   & \\

\#7 ResNet50~\cite{he2016deep} & E & 256$\times$128  &  192 & &   &   &   & \\



\#8 ResNet101~\cite{he2016deep} & R & 256$\times$128  &  128 & 41.24 & 52.98  &  58.89 & 65.53  & 12.04 \\

\#9 ResNet152~\cite{he2016deep} & R & 256$\times$128  &  \red{80} & 42.66 &  54.79 &  60.63 & 66.93  & 12.48 \\
% batch size = 96, CUDA out of memory.

\#10 MobileNetv2~\cite{sandler2018mobilenetv2} & R & 256$\times$128  &  256 & &   &   &   & \\



\#11 Inceptionv3~\cite{Szegedy_2016_CVPR}  & R & 299$\times$299  &  96 &  &   &   &   & \\



\#12 DenseNet121~\cite{huang2017densely} & R & 256$\times$128  &  128 & 39.10 & 50.96  & 56.87  & 62.65  & 09.73 \\
\#12 DenseNet121~\cite{huang2017densely} & G & 256$\times$128  &  128 & \blue{30.63}  &  \blue{42.77}  &  \blue{49.20}  &  \blue{55.69}  & \blue{06.21}  \\
\#12 DenseNet121~\cite{huang2017densely} & E & 256$\times$128  &  128 & 19.25  &  31.31  &  38.04  &  45.63  &  03.11 \\
\#13 DenseNet161~\cite{huang2017densely} & R & 256$\times$128  &  64 & &   &   &   & \\

\#14 DenseNet169~\cite{huang2017densely} & R & 256$\times$128  &  96 & 42.94 & 53.79  & 58.99  & 64.88  & 11.14 \\
      & & & & \red{44.03} & \red{55.15}  & \red{60.11}  & \red{66.41}  & \red{11.59} \\
      \hline
\#15 DenseNet201~\cite{huang2017densely} & R & 256$\times$128  &  64 & 46.62 &  57.19 &  62.64 &  68.28 & 12.24 \\
\hline
\hline
OSNet x1.0~\cite{zhou2021osnet}     & R & 256$\times$128 & 96 & 42.38 & 54.85  & 60.58  & 66.55  & 11.78 \\
OSNet x0.75~\cite{zhou2021osnet}     & R & 256$\times$128 & 160 & 42.96 & 55.13  & 60.45  & 66.20  & 11.13 \\
OSNet x0.5~\cite{zhou2021osnet}     & R & 256$\times$128 & 256 & 41.55 & 54.05  & 59.39  & 65.19  & 10.88 \\
OSNet x0.25~\cite{zhou2021osnet}     & R & 256$\times$128 & 512 & 36.63 & 49.51  & 55.82  &  62.27 & 09.28 \\
\hline
\hline
\#16 ReIDCaps~\cite{huang2019beyond} & R & 224$\times$224  &  \red{20} & 48.55 &  59.94 &  65.26 &  71.18 & 15.34 \\

\#17 2br ResNet50 & R, K & 256$\times$128  &  192 & &   &   &   & \\

\#18 2br ResNet50 & R, E & 256$\times$128  &  96 & &   &   &   & \\

\#19 2br ResNet50 & R, G & 256$\times$128  &  96 &  41.79 & 53.96  & 59.90  & 66.42 & 10.82 \\

\#20 3br ResNet50 & R, G, E & 256$\times$128  &  64 & &   &   &   & \\

\#21 2br DenseNet121 & R, E & 256$\times$128  &  64 & &   &   &   & \\

\#22 2br DenseNet121 & R, G & 256$\times$128  &  64 & &   &   &   & \\

\#23 3br DenseNet121 & R, G, E & 256$\times$128  &  32 & 47.61 &  58.76 &  64.37 & 70.19  & 12.61 \\
    \hline
  \end{tabular}
  }
\end{table}

==> tables/main-results-v20210726-backup-color.tex <==
\begin{table*}[!h]
\tiny
  \caption{Person Re-ID performance comparisons on the test set of \name. Both rank accuracy ($\%$) and mAP ($\%$) are reported. (`R': RGB, `G': grayscale, `E': edge map, `K': body key point, `2br': two branches, `3br': three branches, `mod.': modalities, `dim.': dimensions)}
  \label{main-results}
  \centering
  %\resizebox{\linewidth}{!}{
  \scalebox{1.3}{
  \begin{tabular}{l l l c c c c c c}
    \hline
    
    
\multirow{2}{*}{network/model} & \multicolumn{2}{c}{input} &  \multirow{2}{*}{batch size} & \multicolumn{4}{c}{rank} & \multirow{2}{*}{mAP} \\
\cline{2-3} \cline{5-8}
 & mod. & dim. &   & @1 & @5 & @10 & @20 &  \\
    \hline
    \hline
% vgg13      & & & & \red{} & \red{}  & \red{}  & \red{}  & \red{} \\
% vgg16      & & & & \red{} & \red{}  & \red{}  & \red{}  & \red{} \\
% vgg19      & & & & \red{} & \red{}  & \red{}  & \red{}  & \red{} \\
% \hline
\#1 ResNet18~\cite{he2016deep} & R & 256$\times$128  &  256 & 34.45    &  46.01 & 51.72  & 58.26  &  08.44 \\

\#2 ResNet18~\cite{he2016deep} & G & 256$\times$128  &  256 &  26.61 & 39.02  & 45.45  &  53.06 &  05.49 \\

% ResNet18~\cite{he2016deep} & tri. & 256x128 R & 1e-4, 0.1/40 & 60 & 256 & 38.93 &  53.54 &  59.93 & 66.47 &  09.89 \\

\#3 ResNet34~\cite{he2016deep} & R & 256$\times$128 &  256  & 35.21 &  47.37 &  53.61 &  60.03 & 09.49 \\

\#4 ResNet34~\cite{he2016deep} & G & 256$\times$128  &  256  & 28.60 & 41.53  &  47.98 & 54.87  & 06.39 \\

% ResNet34~\cite{he2016deep} & tri. & 256x128 R & 1e-4, 0.1/40 & 60 & 128 & 38.78 & 52.88 & 59.44 & 66.20 & 10.54 \\

\#5 ResNet50~\cite{he2016deep} & R & 256$\times$128  &  192 & 36.62 & 49.88  &  55.46 & 61.92  & 09.62 \\

\#6 ResNet50~\cite{he2016deep} & G & 256$\times$128  &  192 & 30.04 & 43.12  & 49.82  & 57.04  & 06.96 \\

\#7 ResNet50~\cite{he2016deep} & E & 256$\times$128  &  192 & 16.05 &  28.51 &  35.59  &  43.28 & 03.17 \\

% ResNet50~\cite{he2016deep} & tri. & 256x128 R & 1e-4, 0.1/40 & 60 & 64 & 36.94 & \red{X} & \red{X} & \red{X} & 09.56 \\

resnext50\_32x4d & R & 256$\times$128 & \red{128} & \red{36.94} & \red{48.87}  & \red{54.55}  & \red{60.50}  & \red{10.09} \\
%\hline
wide\_resnet50\_2 & R & 256$\times$128 & \red{128} & \red{33.68} & \red{45.57}  & \red{51.45}  & \red{57.72}  & \red{08.71} \\

\#8 ResNet101~\cite{he2016deep} & R & 256$\times$128  &  128 & 39.31 & 51.65  & 57.36  & 63.72  & 11.00 \\

resnext101\_32x8d & R & 256$\times$128 & \red{64} & \red{40.93} & \red{52.68}  & \red{58.05}  & \red{64.21}  & \red{11.07} \\
%\hline
wide\_resnet101\_2 & R & 256$\times$128 & \red{64} & \red{34.33} & \red{46.46}  & \red{52.42}  & \red{58.69}  & \red{09.03} \\
%\hline
\#9 ResNet152~\cite{he2016deep} & R & 256$\times$128  &  96 & 39.84 & 52.51  & 58.35  &  64.75 & 11.49 \\

\#10 MobileNetv2~\cite{sandler2018mobilenetv2} & R & 256$\times$128  &  256 & 33.71 & 46.51  & 52.72  & 59.45  & 07.95 \\

% MobileNetv2~\cite{sandler2018mobilenetv2} & tri. & 256x128 R & 1e-4, 0.1/40 & 60 & 96 & 36.85 & 51.96 & 58.73  & 65.51 & 09.35 \\
MobileNetv3 Small~\cite{howard2019searching}     & R & 256$\times$128 & \red{768} & \red{28.73} & \red{40.87}  & \red{47.24}  & \red{54.12}  & \red{06.09} \\
MobileNetv3 Large~\cite{howard2019searching}     & R & 256$\times$128 & \red{320} & \red{33.08} & \red{44.99}  & \red{51.32}  & \red{58.14}  & \red{07.56} \\
%\hline
GoogLeNet      & R & 299$\times$299 & \red{96} & \red{29.02} & \red{40.83}  & \red{46.75}  & \red{53.65}  & \red{07.24} \\
\#11 Inceptionv3~\cite{Szegedy_2016_CVPR}  & R & 299$\times$299  &  96 &  35.02 &  47.71 &  53.91 &  60.64 & 08.85 \\

% Inceptionv3~\cite{Szegedy_2016_CVPR}  & tri. & 299x299 R & 1e-4, 0.1/40 & 60 & 32 & 22.18 & \red{X} & \red{X} & \red{X} & 06.01 \\

{\#12 DenseNet121}~\cite{huang2017densely} & R & 256$\times$128  &  128 & 38.26 & 50.27  &  55.91 &  62.40 & 09.12 \\
{\# DenseNet121}~\cite{huang2017densely} & \red{G} & 256$\times$128  &  128 & \red{30.64} & \red{43.02}  & \red{49.41}  & \red{56.44}  & \red{06.14}  \\
{\# DenseNet121}~\cite{huang2017densely} & \red{E} & 256$\times$128  &  128 &  \red{18.21} & \red{30.40}  & \red{36.86}  & \red{44.04}  & \red{02.88} \\
{\#12 DenseNet121}~\cite{huang2017densely} & R & \red{224$\times$224}  &  \red{64} & \red{39.92}  &  \red{51.76}  &  \red{57.21}  &   \red{62.98} & \red{09.99}  \\
% repeat & & & & \red{39.47} & \red{51.05}  & \red{56.76}  & \red{62.72}  & \red{09.86} \\
\#13 DenseNet161~\cite{huang2017densely} & R & 256$\times$128  &  64 & 45.92 &  56.72 & 61.79  & 67.41  & 12.30 \\
% repeat      & & & & \red{45.57} & \red{56.78}  & \red{61.84}  & \red{67.31}  & \red{12.02} \\
\#14 DenseNet169~\cite{huang2017densely} & R & 256$\times$128  &  96 & 43.40 &  54.80 &  60.11 &  65.90 & 11.25 \\

\#15 DenseNet201~\cite{huang2017densely} & R & 256$\times$128  &  64 & 44.98 & 56.13  & 61.32  & 66.98  & 11.71 \\
%\hline
%\hline
shufflenetv2\_x0.5      & R & 256$\times$128 & \red{1024} & \red{17.21} & \red{27.69}  & \red{33.48}  & \red{40.53}  & \red{04.00} \\
shufflenetv2\_x1.0      & R & 256$\times$128 & \red{768} & \red{20.22} & \red{32.95}  & \red{39.58}  & \red{46.89}  & \red{04.60} \\
%\hline
squeezenet1\_0      & R & 256$\times$128 & \red{384} & \red{23.38} & \red{33.17}  & \red{38.64}  & \red{44.34}  & \red{04.78} \\
squeezenet1\_1      & R & 256$\times$128 & \red{640} & \red{23.52} & \red{33.54}  & \red{39.26}  & \red{45.59}  & \red{05.02} \\
%\hline
mnasnet0\_5 & R & 256$\times$128 & 512 & \red{17.52} & \red{29.17}  & \red{36.20}  & \red{43.51}  & \red{02.79} \\
mnasnet1\_0 & R & 256$\times$128 & \red{256} & \red{30.63} & \red{44.02}  & \red{50.40}  & \red{57.56}  & \red{06.25} \\
\hline
SCNet50~\cite{liu2020improving}      & R & 256$\times$128 & \red{160} & \red{35.07} & \red{47.73}  & \red{54.32}  & \red{60.73}  & \red{09.53} \\
SCNet50\_v1d~\cite{liu2020improving}      & R & 256$\times$128 & \red{128} & \red{37.46} & \red{50.20}  & \red{56.13}  & \red{62.36}  & \red{09.42} \\
SCNet101~\cite{liu2020improving}      & R & 256$\times$128 & \red{96} & \red{37.25} & \red{50.09}  & \red{56.28}  & \red{63.16}  & \red{10.35} \\
\hline
%\hline
OSNet ibn x1.0~\cite{zhou2021osnet} & R & 256$\times$128 & \red{96} & \red{42.75} & \red{54.91}  & \red{60.82}  & \red{66.80}  & \red{10.97} \\
OSNet x1.0~\cite{zhou2021osnet}     & R & 256$\times$128 & 96 & \red{39.65} & \red{52.22}  & \red{58.32}  & \red{64.23}  & \red{10.34} \\
OSNet x0.75~\cite{zhou2021osnet}     & R & 256$\times$128 & 160 & \red{39.96} & \red{51.89}  & \red{57.69}  & \red{63.85}  & \red{09.92} \\
OSNet x0.5~\cite{zhou2021osnet}     & R & 256$\times$128 & 256 & \red{38.09} & \red{51.08}  & \red{56.79}  & \red{63.27}  & \red{09.59} \\
OSNet x0.25~\cite{zhou2021osnet}     & R & 256$\times$128 & 512 & \red{34.94} & \red{47.70}  & \red{54.10}  & \red{60.77}  & \red{08.62} \\
%OSNet & CE & 256x128 & 1e-4, 0.1 per 20 & 30 & 96 & 0.4464 & 0.5680 & 0.6247 & 0.6806 & 0.1100 \\
\hline
BNNeck Re-ID Res18~\cite{luo2020strong}     & R & 256$\times$128 & \red{224} & \blue{38.17} & \red{51.93}  & \red{58.08}  & \red{64.70}  & \red{09.51} \\
BNNeck ResNet34~\cite{luo2020strong}     & R & 256$\times$128 & \red{128} & \red{40.06} & \red{53.49}  & \red{59.55}  & \red{66.25}  & \red{10.52} \\
BNNeck ResNet50~\cite{luo2020strong}      & R & 256$\times$128 & \red{56} & \red{47.45} & \red{59.47}  & \red{65.19}  & \red{71.10}  & \red{12.98} \\
\hdashline
BNNeck ResNet50~\cite{luo2020strong}      & G & 256$\times$128 & \red{56} & \red{4002} & \red{5404}  & \red{6019}  & \red{6709}  & \red{0943} \\
BNNeck ResNet50~\cite{luo2020strong}      & E & 256$\times$128 & \red{56} & \red{2175} & \red{3599}  & \red{4311}  & \red{5081}  & \red{0367} \\
2br BNNeck ResNet50~\cite{luo2020strong}      & R, G & 256$\times$128 & \blue{28} & \red{46.62} & \red{59.72}  & \red{65.58}  & \red{71.48}  & \red{13.12} \\
BNNeck ResNet50~\cite{luo2020strong}      & R, G, E & 256$\times$128 & \red{56} & \red{} & \red{}  & \red{}  & \red{}  & \red{} \\
\hdashline
BNNeck ResNet101~\cite{luo2020strong}     & R & 256$\times$128 & \red{40} & \red{48.10} & \red{60.70}  & \red{66.10}  & \red{72.06}  & \red{13.72} \\
BNNeck ResNet152~\cite{luo2020strong}     & R & 256$\times$128 & & \green{50.29} & \red{62.27}  & \red{67.85}  & \red{73.63}  & \green{14.59} \\
BNNeck Re-ID Den121     & R & 256$\times$128 & & \green{4786} & \red{6047}  & \red{6588}  & \red{7164}  & \green{1341} \\
\hline
\tabincell{c}{\#16 ReIDCaps~\cite{huang2019beyond}\\ (full model)} & R & 224$\times$224  &  24 & 44.29 & 56.44  & 62.01  & 68.01  & 13.25 \\
% repeat & & & & \red{44.49} & \red{56.32}  & \red{61.80}  & \red{68.21}  & \red{13.28} \\
% repeat  & & & & \red{44.97} & \red{56.35}  & \red{61.99}  & \red{68.01}  & \red{13.29} \\
% repeat  & & & & \red{43.88} & \red{56.18}  & \red{61.98}  & \red{67.77}  & \red{13.03} \\
\tabincell{c}{\#16 ReIDCaps~\cite{huang2019beyond}\\ (full model, resnet50 backbone)} & R & \red{224$\times$224}  &  \red{32} & \red{3949} & \red{5228}  &  \red{5868} & \red{6499}  & \red{1133} \\
   \hline
\tabincell{c}{\#16 ReIDCaps~\cite{huang2019beyond}\\(no auxiliary module\&loss)} & R & 224$\times$224  &  24 & \red{35.41} & \red{46.66}  & \red{52.09}  & \red{58.13}  & \red{09.25} \\
% repeat & & & & \red{34.97} & \red{46.23}  & \red{51.80}  & \red{58.26}  & \red{09.33} \\
 \hline
\tabincell{c}{\#16 ReIDCaps~\cite{huang2019beyond}\\ (no capsule module\&loss)} & R & \red{224$\times$224}  &  80 & \red{39.38} & \red{51.86}  & \red{57.82}  & \red{64.44}  & \red{11.16} \\
% repeat & & & & \red{39.94} & \red{52.22}  & \red{57.73}  & \red{64.14}  & \red{11.36} \\
%\#16 ReIDCaps~\cite{huang2019beyond} & R & \red{256$\times$128}  &  24 & \red{x} & \red{x}  & \red{x}  & \red{x}  & \red{x} \\
\hline
\#17 2br ResNet50 & R, K & 256$\times$128  &  192 & 36.53 &  48.87 &  54.86 &  61.47 & 09.54 \\

\#18 2br ResNet50 & R, E & 256$\times$128  &  96 & 40.26 & 52.91  & 59.11  & 65.47  & 10.43 \\

\#19 2br ResNet50 & R, G & 256$\times$128  &  96 & 40.52 &  53.65  &  59.61 &  65.60 & 10.22 \\

\#20 3br ResNet50 & R, G, E & 256$\times$128  &  64 & 41.67 & 54.28  & 60.04   &  66.37 & 11.03 \\

\#21 2br DenseNet121 & R, E & 256$\times$128  &  64 & 44.55 & 56.40  &  62.03 &  67.85 & 11.21 \\

\#22 2br DenseNet121 & R, G & 256$\times$128  &  64 & 44.80 &  56.79 &  62.48 & 68.06  & 11.36 \\
\hline
\#23 3br DenseNet121 & R, G, E & 256$\times$128  &  32 & 45.36 & 57.36  & 62.91  & 69.29  & 11.73 \\
%  repeat & & & & \red{44.87} & \red{57.14}  & \red{63.12}  & \red{69.26}  & \red{11.36} \\
%  repeat & & & & \red{45.36} & \red{57.36}  & \red{62.91}  & \red{69.29}  & \red{11.73} \\
%  repeat & & & & \red{44.75} & \red{56.80}  & \red{62.60}  & \red{68.34}  & \red{11.54} \\
%  repeat   & & & & \red{46.00} & \red{58.24}  & \red{63.80}  & \red{69.61}  & \red{11.76} \\
%  repeat    & & & & \red{45.06} & \red{57.66}  & \red{63.32}  & \red{69.30}  & \red{11.86} \\
%  repeat     & & & & \red{46.09} & \red{58.43}  & \red{63.77}  & \red{69.85}  & \red{11.87} \\     
%  repeat    & & & & \red{} & \red{}  & \red{}  & \red{}  & \red{} \\
    \hline
    \hline
%ViT B16~\cite{dosovitskiy2020image} & R & \red{224$\times$224} & 128 4GPUs & \red{38.90} & \red{50.79} & \red{56.25} & \red{62.47} & \red{11.11} \\ 
ViT B16~\cite{dosovitskiy2020image} & R & \red{256$\times$128} & 128 4GPUs & \red{41.30} & \red{53.83} & \red{59.44} & \red{65.44} & \red{12.04} \\ % ImageNet21K, class token,
      & R & & 64 1GPU & \red{43.96} & \red{55.82}  & \red{61.22}  & \red{66.74}  & \red{12.98} \\ %    ImageNet21K, class token,  learning rate decay changes.
            & R & & 64 1GPU & \red{49.78} & \red{61.81}  & \red{67.38}  & \red{72.92}  & \red{14.98} \\ % ImageNet21K+ImageNet1K, mean tokens, no layer norm,
                  & Gray & & 64 1GPU & \red{38.93} & \red{51.94}  & \red{58.50}  & \red{65.12}  & \red{10.43} \\ % ImageNet21K+ImageNet1K, mean tokens, no layer norm,
%      & Gray & & 64 1GPU & \red{} & \red{}  & \red{}  & \red{}  & \red{} \\ %ImageNet21K+ImageNet1K, mean tokens, +layer norm,
\hline
ViT B16 0.3* Gray+1* RGB    & R, G & \red{256$\times$256} & 64 1GPU  & \red{0.4725} & \red{0.5852} & \red{0.6366} & \red{0.6936} & \red{0.1470} \\ % 3* Gray+1* RGB
ViT B16 0.3* Gray+0.7* RGB    & R, G & \red{256$\times$256} & 64 1GPU & \red{0.4724} & \red{0.5853} & \red{0.6407} & \red{0.6953} & \red{0.1463} \\ % 0.3* Gray+0.7* RGB
\hline
DeiT     & R & 256$\times$128 & 64 1GPU & \blue{0.4443} & \blue{0.5625} & \blue{0.6182} & \blue{0.6746} & \blue{0.1372} \\
%DeiT      & & & & \red{} & \red{}  & \red{}  & \red{}  & \red{} \\
    \hline
  \end{tabular}
  }
\end{table*}

==> tables/unsupervised-results.tex <==
\begin{table}[!t]
  \caption{Unsupervised results.}
  \label{unsupervised-results}
  \centering
  \resizebox{0.5\linewidth}{!}{
  \begin{tabular}{l l l l l l}
    \hline
    
    
\multirow{2}{*}{method/model} &  \multicolumn{4}{c}{rank} & \multirow{2}{*}{mAP} \\
\cline{2-5}
    & @1 & @5 & @10 & @20 &  \\

    \hline
    \hline
\#1  xx & xx & xx & xx & xx & xx \\    
\#2  xx & xx & xx & xx & xx & xx \\
\#3  xx & xx & xx & xx & xx & xx \\
\#4  xx & xx & xx & xx & xx & xx \\
\#5  xx & xx & xx & xx & xx & xx \\
\#6  xx & xx & xx & xx & xx & xx \\
%\#7  xx & xx & xx & xx & xx & xx \\
    \hline
  \end{tabular}
  }
\end{table}
